Stein Variational Inference for Discrete Distributions

Gradient-based approximate inference methods, such as Stein variational gradient descent (SVGD), provide simple and general-purpose inference engines for differentiable continuous distributions. However, existing forms of SVGD cannot be directly applied to discrete distributions. In this work, we fill this gap by proposing a simple yet general framework that transforms discrete distributions to equivalent piecewise continuous distributions, on which the gradient-free SVGD is applied to perform efficient approximate inference. The empirical results show that our method outperforms traditional algorithms such as Gibbs sampling and discontinuous Hamiltonian Monte Carlo on various challenging benchmarks of discrete graphical models. We demonstrate that our method provides a promising tool for learning ensembles of binarized neural network (BNN), outperforming other widely used ensemble methods on learning binarized AlexNet on CIFAR-10 dataset. In addition, such transform can be straightforwardly employed in gradient-free kernelized Stein discrepancy to perform goodness-of-fit (GOF) test on discrete distributions. Our proposed method outperforms existing GOF test methods for intractable discrete distributions.

==> tex/Rebuttal.tex <==
\onecolumn
\section{AnonReviewer2: Overall a good paper}
This paper presents a sampling framework for discrete distribution based on gradient-free Stein variational gradient descent. It exploits a continuous proposal distribution and a map which map the sampled continuous random variable to the discrete one. When the map evenly partition the continuous space, then the construction is shown to be an exact continuous parameterization of the original discrete one. Experiments on Ising model, Bernoulli RBM and binarized neural networks are done to verify the effectiveness of the proposed method. 
      
      Strength:
      
      1, The idea of extending gradient-free Stein variational gradient descent to the discrete distributions is interesting. 
      
      2, Experiments cover quite a few of different classes of models which are compelling.
      
      3, The paper is clearly written and easy to follow. 
      
      Weakness & Suggestions:
      
      1, It would be great to consider more structured discrete object where the evenly partition may be challenging since almost all experiments in the paper just uses sign function. For example, you can consider the distributions over trees. Showing how to instantiate your framework under these settings will strengthen the paper.
      
      {\bf Thanks! Our method works naturally for multi-class categorical distributions as shown in Figure 2. We will perform more experiments on non-binary graphical models in the reivision.}
      
      2, Using MMD as the evaluation metric is not that satisfying as it highly depends on the chosen kernel and its hyperparameters. It would be great to provide other metrics.
      
      {\bf Thanks for your suggestion. We did report the MSE for mean estimation for Ising model and UAI instances (/Figure 3-4). We added mean square error metric for the RBM experiment and found it also significantly outperforms Gibbs and DHMC. We put it in our revision.  \red{There should no way to upload figures }}
      
\begin{figure}[h]
\centering
\begin{tabular}{cc}
\includegraphics[height=0.2\textwidth]{figs/rbm_mse_sam.pdf} &
\includegraphics[height=0.2\textwidth]{figs/rbm_mse_dim.pdf} \\
{\small (a)  Fix dimension} &
{\small (b)  Fix sample size} 
\end{tabular}
\caption{\small Bernoulli RBM with number of visible units $M=25$. In (a), we fix the dimension of visible variables $d=100$ and vary the number of samples $\{\vz^j\}_{j=1}^n$. In (b), we fix the number of samples $n=100$ and vary the dimension of visible variables $d$. We calculate the MSE for estimating the mean $\E[z]$ (lower is better).}
\label{fig:rbm}
\end{figure}
      
      3, It would be very interesting to see whether this method could help the learning of energy based model, especially the generative models.
      
      {\bf Thanks for the suggestion. It is an interesting direction. It is straightforward to incorporate our new inference algorithm in standard learning methods such as MLE and contrastive divergence. We leave this to future work.}
      
      Minor:
      
      The probability distribution in step 1) of algorithm 1 should be proportional to not equal to the construction.
      
     {\bf Thanks for pointing out this typos. We revised it.}
      
      Overall, I like the idea and recommend accept.
      
Rating:  7: Good paper, accept
Confidence:  3: The reviewer is fairly confident that the evaluation is correct.      


\section{AnonReviewer1: SVGD for discrete distributions}
The authors propose applying SVGD to approximate expectations with respect to discrete distributions.  This is accomplished by replacing the discrete with a continuous analog and the applying the standard SVGD method.  The way the continuous analogs are constructed is by choosing simple continuous distributions, constructing a uniform partitioning of this distribution, and then multiplying by the appropriate weight.  The paper concludes with a variety of experiments comparing the proposed approach against Gibbs sampling.  The paper, though easy to follow, has a number of typos that make it irritating to read but do not impede understanding.
      
      Specific comments:  
      
      1)  The novelty of the approach seems somewhat limited as it is a simple application of existing methods.  In particular, the work could be strengthened if the continuous analog were chosen is some more meaningful way.  As it stands, there are an infinite number of possible continuous representations and the authors provide no mechanism for choosing between them.
      
      {\bf A key limitation of SVGD is that it only applies to continuous variable models, and it was a main open question to extend it to discrete variables. The idea addressing this important problem using our construction of surrogate distribution is only obvious in hindsight. Although there are many possible continuous surrogate, our construction is particularly simple, straightforward and computationally efficient. We will further investigate more advanced strategies for adaptively improving the continuous surrogate, but we would like to argue that a key advantage of our current method is its simplicity and effectiveness.}
      
%      {\bf   We thank the reviewer for the comments. We propose a new algorithm to sample from the discrete distributions where the original SVGD and gradient-free SVGD cannot be applied. We propose a simple yet powerful transformation, quantile transformation, to a transformed piecewise continuous target distribution where the efficient differentiable surrogate distribution is easy to construct. Leveraging the power of annealed importance sampling and annealed GF-SVGD (bridging between any initial proposal and the target to construct effective importance weight), any kind of continuous representations will be effective when applying annealed GF-SVGD. In particular, we propose a simple to calculate yet powerful continuous representation which can be widely applied to a range of discrete probability models.}
      
      2)  The comments at the end of section 3 are hard to follow.  If the continuous representation is not differentiable, then the gradient-free SVGD cannot be applied.  The authors suggest that you can approximate the continuous representation, but it is unclear how one computes smooth approximations of these functions (again, there could be many and the authors offer no help here).
      
      {\bf We rewrite section 3 to make it easy to read. 
      We don't need to compute the gradient of the continuous representation. Our goal is not using the surrogate to approximate the piecewise continuous target. We only need to leverage the gradient of the surrogate distribution with importance weight when applying gradient-free SVGD. The smooth surrogate we construct is easy to compute based on formula (12), (14), (16).}
      
      3)  The experiments need to have error bars as these are the results of running a sampling procedure.
      
      {\bf We calculate the mean square error (square of bias plus variance) between the estimator and the ground-truth quantity of interest, which already reflects the error bars (variance).}  
      
      
      4)  What is the practical running time of the different methods in the NN case.  Maybe some of the other methods can be run with more ensembles in the same amount of time it takes to do the proposed method?
      
      {\bf When applying our learned model to predict the accuracy on test data, the running time of ours, BAG and BENN(Adaboost) is the same since all three methods just linearly average the learned models with same NN size.}

Rating:  4: Ok but not good enough - rejection\\
Confidence:  4: The reviewer is confident but not absolutely certain that the evaluation is correct.

\section{AnonReviewer4:Interesting idea but no theory}
The paper provides a way to approximate integrals with respect to a discrete measure by iteratively updating "particles" using SVGD applied to a continuous surrogate. Although the idea is interesting, there is no theory to guide practice. For instance, in Algorithm 1 of the paper what is epsilon and how should one tune it in practice. How does it effect the performance? Also, how does the approximation error scale with the "sample size" n? What else does the approximation error depend on?

{\bf   We thank the reviewer for the comments. Our sampling algorithm for discrete distribution inherits most theoretical property from SVGD. The epsilon and others are hyperparameters appearing in standard algorithms. 
For all the experiments we have done in this paper, the setting where epsilon equals 1e-4 with Adam optimizer works well. Based on the theory of SVGD, the mean square errors scale O(1/n), which we empirically demonstrate on binary Ising model and Bernoulli restricted Boltzmann machine.}

Rating:  4: Ok but not good enough - rejection
Confidence:  3: The reviewer is fairly confident that the evaluation is correct

\section{AnonReviewer3:interesting paper, some concerns on the experimental evaluation}
The paper proposes an approach to transform discrete distributions to a distribution with piecewise continuous pdf. This transformed distribution is then utilized to perform approximate inference using Gradient-Free SVGD with a surrogate continuous distribution. Experimental results demonstrate applications such as sampling, inference on Ising model / Boltzmann machines, as well as “posterior inference” on binary neural networks.
      
      Pros:
      
      The experimental results are impressive, and the method seems promising over multiple applications, such as sampling and training ensembles of binarized neural networks.
      In Discrete HMC the transformation is from discrete to step functions over energy functions, and here it is from discrete to general piecewise continuous distributions. This more general transformation could be applied in other settings.
      
      Cons and questions:
      
      The main contribution here is the transformation from discrete probabilities to a piecewise continuous pdf. It seems that the performance of the method would depend heavily on the choice of piecewise continuous distributions and differentiable surrogate, and the experiments do not contain ablations over alternative approaches (such as simply using stepwise pdf). 
      For example, I suspect that if one chooses a poor Gamma(x) (e.g., applying some kind of random permutation that destroys the underlying structure of the discrete space), performance would be extremely poor. An ablation study on the effect of these choices seem very important, given that this is the main contribution of this paper.
      
      {\bf   We thank the reviewer for the comments. We agree that the choice of differentiable surrogate is important for the practical performance. Figure 1 in GF-SVGD provides an ablation study to the choice of surrogate distributions. Basically, it indicates that we should choose surrogate distributions with wide variance. While it might be challenging to choose an effective surrogate in continuous distributions, it is interesting to observe that it is easy to construct an effective surrogate on discrete distributions such as categorical distribution (Figure 1) and binary Ising model, Bernoulli restricted Boltzmann machine and Binarized NN. Starting from a poor surrogate, we can apply annealed GF-SVGD to evolve along a bridge of intermediate distributions between the initial surrogate and the target to ensure the effectiveness of our sampling algorithm.}
      
      On this note, Algorithm 1 is not really an algorithm - no explicit procedure is given for computing the needed pieces. I suggest to rewrite it, making it clear what the user needs to provide as input, and what the algorithm will provide as an output. You should also be explicit about the fact that these choices made by the user will affect performance.
      
      {\bf Thanks for your suggestions. We will emphasize input/output in Algorithm 1 of our revised version.}
      
      I have some questions about the experiments:
      
      - it is surprising that the method does better than exact monte carlo (i assume that means exact i.i.d. samples from the true underlying distribution). is it because the samples from SVGD are not i.i.d?
      
      {\bf The samples in SVGD are not i.i.d. and interacting with each other at each iteration. The fact that the samples in SVGD is more efficient than that of exact Monte Carlo has been demonstrated in original SVGD and several extensions.}
      
      - what is the performance is you attempt to estimate more complex marginals, for example pairwise ones?
      
      - when you compare to Gibbs sampling, are you using just the final sample ("to take the last sample of each chain") or the entire chain (after burn-in)? using the final sample does not seem to be a fair comparison
      
      We compare with Gibbs sampling using the final samples since we use the same number of iterations for all methods (the number of iterations in Gibbs sampling is calculated after burn-in steps.)
      
      - no information is given on the runtime of the proposed method. to be fair to gibbs, you should compare them for the same amount of wall clock time
      
      {\bf Besides discrete graphical probability models (Ising model, Bernoulli RBM and BNN), we will add some more complex and interesting application in our revision. As the number of iterations in Gibbs sampling is counted after burn-in steps, our method will need less iteration in total. Within each iteration, Gibbs sampling will also iterate over each coordinate. Therefore, our method is faster in terms of running time in Ising model and Bernoulli RBM.}
      
      - why was DHMC not tested on the Ising model experiment?
      
      {\bf As we compared two baselines (exact Monte Carlo and Gibbs sampling), we didn't add it in original draft. We add DHMC to Binary Ising model like we did in Bernoulli RBM in our revised version.}
      
      - how was the RBM trained? via contrastive divergence?
      
      {\bf In our setting, we don't need to train a RBM model. Our goal is to sample from a given Bernoulli RBM distribution.}
      
      There are numerous typos throughout the paper. 
      
      {\bf We carefully revised typos.} 

Rating:  5: Marginally below acceptance threshold.\\
Confidence:  4: The reviewer is confident but not absolutely certain that the evaluation is correct 

\section{AnonReviewer5: Extension of Stein variational gradient descent to discrete setting}
Summary. This work proposes an extension of SVGD (Liu+, 2016) with respect to the discrete setting. A set of experiments are given comparing the proposed method against Gibbs sampling. Though interesting, the current approach is a somewhat straightforward application of existing methods. 

{\bf We thank the reviewer for the comments. We propose a new algorithm to sample from the discrete distributions where the original SVGD cannot be applied. We design the quantile transformation to transform the discrete ones to a corresponding piecewise continuous distribution. The advantages of such design are that it is convenient to construct an efficient surrogate when applying GF-SVGD and it is easy to calculate each term in the update even in high dimensions. }



==> tex/Rebuttal_AISTATS.tex <==
\section{Review 1}
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This paper presents a new posterior inference method for discrete distribution, which extends SVGD and GF-SVGD.

The contributions of the paper are as follows:

1. The paper proposes a way to transform discrete distributions into continuous distributions, then the inference of the continuous ones can be done by SVGD and GF-SVGD.

2. With the proposed transformations, the goodness of fit testing of discrete distributions can be computed according to the kernelized Stein discrepancy, which is reported to be a better measure than MMD and DKSD.
2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
Strengths:

1. The paper is well written and easy to follow.

2. The proposed idea is simple yet effective.

3. The experimental results are relatively comprehensive.

Weakness:

1. My first concern is that if we consider a boarder area of posterior inference for discrete distributions, there are many other inference methods other than SVGD, such as REENFORCE, gumbel-softmax, ... In the experiments, the paper only compares with Gibbs and DHMC. Therefore, it is hard to evaluate how the proposed method is compared with many others, which may limit the applications of the proposed method. So it is suggested to compare with some other methods in this area. Moreover, it might be also interesting to compare with the Stein Variational Policy Gradient [1], which may also be applied to inference for discrete distributions

2. Another concern is on GF-KSD with the proposed transformations. Although it is shown to be more consistent than MMD and DKSD, it is unclear if the proposed one can be generalised to measure other models than the proposed one. Note that measurements like MMD can be used in general cases.

[1] Liu, Y., Ramachandran, P., Liu, Q. and Peng, J., 2017. Stein variational policy gradient. arXiv preprint arXiv:1704.02399.

3. [Score] Please provide an overall score for the submission.
Accept: Good paper

4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
None

5. [Review Summary] Please enter a 1-2 sentence summary of your review explaining your overall score.
I think the idea is intuitive and the experiment results look promising.

6. [Reproducibility] Are the experiments (if present) detailed enough to allow reproducibility?

I think the paper has a relatively good reproducibility as the experimental settings are described in detail. But it is also suggested to release the code.

7. [Code] Was the code made available by the authors?
No

{\bf Reply:} We thank the reviewer for critical, supportive, and insightful comments!

Thanks for pointing out the comparison with other baselines. We are implementing a recently proposed framework[1](particle-based variational methods for discrete models), which is most relevant to ours. As our method is based on SVGD, which shows more efficiency than particle-based mirror descent[2], our method provides a promising variational tool for discrete models. We will also compare ours with gumbel-softmax methods, which is proposed for optimization and not mainly used for sampling and cannot provide consistent estimation as there is a bias between the approximate model and the target distribution. In this case, our method will provide more consistent result compared with gumbel-softmax methods. As online codes for these methods are not online available, we are contacting the authors and will add the results in our final version. 

SVPG is proposed to solve discrete optimization (optimizing the policy, etc.), which is different from our discrete sampling goal in this paper. We will cite it and discuss such difference in our next version. 

Our GF-KSD can also be applied to general discrete distributions, where the paper only provides two widely-used discrete models due to space limit. We consider applying our GF-KSD to some more interesting models such as the LDA model suggested by Review 2. We will release our code upon acceptance.

[1] Ardavan Saeedi, Tejas D. Kulkarni, Vikash K. Mansinghka and Samuel J. Gershman , Variational Particle Approximations, JMLR 2017.

[2] Bo Dai, Niao He Hanjun Dai and Le Song, Provable Bayesian Inference via Particle Mirror Descent, AISTATS 2016.

\red{[I think you should say that something like SVPG can be used to solve discrete optimization, but optimizing the policy, etc]}. 

\section{Review 2}
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This paper introduces an approach for extending stein variational gradient descent to discrete distributions. It is based on a two-step idea: first, replace the discrete domain with a continuous relaxation. Then, use an importance-weighted kernel Stein discrepancy, targeting the continuous relaxation, with an appropriate importance sampling proposal. This obviously depends then on the quality of both the relaxation and the proposal; however, some guidelines are given, and experimental results are promising.
2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
Strengths:

Overall I thought the paper was well organized, with the description of continuous parameterizations clearly presented and gave a good intuition for how they are usable for Algorithm 1.

The method is an extension of methods which are based on an importance-weighted (or here "gradient free") KSD, and as such inherits any theoretical justifications and intuitions for understanding performance.


Weaknesses:

It seems like how well this will work depends a lot on whether or not a suitable surrogate $\rho$ can be found. The suggestion in the "simple" cases, or using $p_0$, does not seem like it could be reliably extended to more complex data (e.g. non-ordinal distributions, or discrete distributions with sparse probabilities, or combinatorial spaces). Indeed, the experiments for the RBM and binarized neural network require using a relaxation of the sign function — in this case it is fairly straightforward, but I don't know how well this works in general. (See later question.)

I'm also not convinced the performance is *that* good. For example, for the ising model it is stated "as $|\sigma_p|$ increases, the difficulty increases". The high gains of performance are shown for the "easy" setting, i.e. "as $\sigma_p \rightarrow 0$, our method significantly outperforms MC and Gibbs sampling". — so, this means that it works very well (faster than sampling!) but in a most pronounced manner on the "easy" cases. In general I am not too concerned, but simply cautious. 

\red{For the Bayesian neural network (i.e. the bernoulli RBM), I would have liked to see a comparison with some other variational inference approach.}

There are many typos and spelling mistakes throughout the paper, too many to list here. This paper needs to be proofread before the final version, but in all honestly papers should be proofread *prior to submission*. Running at least basic spellchecker should be a prerequisite to submitting to a conference.

3. [Score] Please provide an overall score for the submission.
Weak Accept: Borderline, tending to accept

4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.

What is going on with the blue dashed lines in figure 2? I don't understand why the heights are different in 2(c) and 2(d) — according to the caption, these are even mixtures of 5 gaussians. Why are they different heights? What are we looking at here?

Would this approach work on topic models like LDA? What sort of continuous relaxation makes sense for categorical variables which do not have an ordinal interpretation, and are non-binary, and possibly sparse? This is a very different setting from either the categorical example in the paper, or from the examples with +/- 1 as discrete values.

Is there a different variational inference method that should be considered as a more realistic baseline for the Bernoulli RBM example? The MCMC methods are great for establishing ground truth, but (though I am not too familiar with the setting) I am skeptical they represent common practice.

Fix all spelling errors and typos.

{\bf Reply:} We thank the reviewer for critical, supportive, and insightful comments! 

Our method can be effectively applied to the structured discrete models, which can be easily leveraged to construct the surrogate as shown in binarized neural network and Bernoulli RBM. It will be interesting to extend our method to non-structured discrete models(non-ordinal distributions, or discrete distributions with sparse probabilities, or combinatorial spaces). 

We vary the choice of $\sigma_p$ where the difficulty of the inference task increases as $|\sigma_p|$ increases. We can see from Fig. 3 that our method consistently outperforms the vanilla Monte Carlo and Gibbs sampling. We will use more concrete descriptions when comparing our method with other baselines in Ising model experiment. 

The blue line in Figure 2 is the surrogate distribution (base function), which is induced from the derivative of the transform F(x). The base function as illustrated in caption of Figure 2 is the Gaussian mixture model with five components. The reason why the base function has different heights in different components of GMM is that the weight for each Gaussian component in GMM is different. We investigate different choices of the transform (base function), as illustrated in Section 4.2. We explore different choices of the base functions and suggests that the Gaussian base function is a simple yet effective choice for constructing the transform. 

Thanks for suggesting other important applications! It is interesting to see the performance of our method in LDA and we leave it to our further experiments. 

We are comparing our method with a recently proposed particle-based variational framework for discrete models[1] on Ising model and Bernoulli RBM, which is most relevant to ours. As the online codes of their methods are not available, we need to add the results in our next version. Our method inherits the merits of the recently proposed SVGD framework, which converges faster and has better sample efficiency than particle-based methods[2]. 

We will also fix the typos in the draft and very much appreciate finding these out.
 
\red{just ignored the comments on comparison with VI?}

\section{Review 3}
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This paper tackles the problem of performing efficient and accurate probabilistic inference of high-dimensional discrete distributions. Existing approximate inference methods, such as Gibbs sampling and Metropolis-Hastings algorithms, suffer from either slow convergence or inacurracy. The recently proposed Stein variational gradient descent (SVGD) allows fast convergence with theoretical asymptotical guarantees, and has a gradient-free variant (denoted GF-SVGD), but applies to continuous distributions only.

In this work, the authors develop an approximate inference framework specifically designed for discrete distributions, and which consists in: (i) constructing a piecewise continuous distribution and a map, from which we can retrieve the discrete distribution, (ii) constructing a differentiable surrogate of this piecewise continuous distribution, (iii) applying GF-SVGD, and (iv) retrieving the associated discrete distribution.

The main contributions can then be summarized as follows:
- Development of a new approximate inference framework for discrete distributions and adapted to high-dimensional settings.
- Development of a new method for goodness-of-fit test between discrete distributions, based on this framework.
- Extensive empirical evaluation of these two techniques on several models and comparison to the state-of-the art.

2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
Strengths:
- The paper is well-written and very clear.
- The topic is relevant. In particular, I found the goodness-of-fit test method as well as the application to the task of training Binarized Neural Network extremely useful.
- The experiment section is quite extensive and interesting: the method is tested on various problems, including complex high-dimensional settings with neural networks, and the empirical results clearly show that the proposed approximate inference method is accurate and the goodness-of-fit method is able to make more meaningful comparisons than DKSD and MMD.

Weaknesses:
- In my opinion, it would be relevant to compare the goodness-of-fit method to the optimal transport divergences, now very popular in the field of statistical inference.
- Some imprecision: I don't understand why in Fig.2 the green bars are at -1, -0.5, 0, 0.5, 1 while in the legend it says that $p_*$ takes values in -2, -1, 0, 1, 2. Also, for further clarity, it would suggest to plot $p_*$ on Fig. 2b,c,d.

Minor comments: The paper contains some typos, as listed below.
- Introduction: "In particular, our algorithm is shown to be provide a promising tool", "for ensemble learn of binarized neural network (BNN) in whichs", "non-differentialbe"
- Under Eq.4: not the same font for 'D' (should be $\mathcal{D}$)
- Under Eq.6: "which does not depends"
- Last paragraph of Section 2: "on discret distribution"
- 1st paragraph of Section 3: "We first provides"
- Paragraph "Constructing Continuous Parametrizations": "it is difficult to quantitatively the notation of difficulty"
- Before Definition 3: "a map $\Gamma$ that evenly partition[s]"
- Paragraph "Bootstrap Sample": "The asymptotic distribution of ... under the hypothesis cannot be evaluated", what hypothesis? + please define $\alpha$.
- Paragraph "Bernoulli Restricted Boltzmann Machine": "Fig. 4(b) shows that the performance of our method is [the] least sensitive"
- Section 4.4: the sentence "Learning the target probability model is framed as drawing n samples..." is written twice.

3. [Score] Please provide an overall score for the submission.
Accept: Good paper

4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
It would be nice if the authors could clarify (i) how the goodness-of-fit method compares to the optimal transport divergences, for example the Wasserstein metric (e.g., with empirical results such as in Fig. 5), and (ii) whether the even partition can be obtained via clustering instead of relying of the quantiles (which cannot be available or inaccurate with a limited set of samples).

5. [Review Summary] Please enter a 1-2 sentence summary of your review explaining your overall score.

The proposed approximate inference method and associated goodness-of-fit test techniques are well motivated and clearly explained. The experiment section clearly show their empirical advantages.

6. [Reproducibility] Are the experiments (if present) detailed enough to allow reproducibility?
Yes: The code was not provided, but the main paper and supplementary material contain a lot of implementation details.

{\bf Reply:} We thank the reviewer for critical, supportive, and insightful comments! 

We consider adding a variational baseline[1] to the Bernoulli RBM experiment and will update it in our next version. The merit of KL divergence is that the variable transform has closed-form solution while other divergences such as Wasserstein metric does not, which casts a challenging optimization problem. We will compare ours with Wasserstein metric-based variational method[3], which requires the Sinkhorn iterations, in next version.

Thanks for pointing out the typos that the green bars in Fig. 2 take values at -1, -0.5, 0, 0.5, 1 while in the caption it says values -2, -1, 0, 1, 2. We will fix our caption to be consistent. As Fig. 2(b, c, d) x axis has much larger range. The values -1, -0.5, 0, 0.5, 1 in green bars will be close and difficult to recognize. We use same $p_*$ for (a,b,c,d) and only plot in (a) in our current version. We will also plot $p_*$ for (b,c,d) in next version.

We will also fix the typos in the draft and very much appreciate finding these out. We will release our code upon acceptance.

[3] Luca Ambrogioni et al. Wasserstein Variational Inference, arxiv.org:1805.11284.pdf 

\red{Need some more serious comments on comparison with optimal transport distance.}

==> tex/ST_estimator.tex <==
\section{Surrogate Model As Control Variates for Training Stochastic BNN}
Let $\bd{W}=\{\bd{W}_i\}_{i=1}^L$ be the binary weight of BNN. The loss function is 
\begin{equation*}
L(\bd{W})=\E_X[\E_{\pi_{\bd{\theta}}(\bd{W})}[f(\bd{W}, X)]]=\E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(H(\bd{Z}), X)]],    
\end{equation*}
where $\bd{W}=H(\bd{Z})=1$ if $\bd{Z}>0$ else $\bd{W}=H(\bd{Z})=-1.$

Let $\bd{Z}=\bd{\mu}+\bd{\sigma}\epsilon.$ Let $S$ be the soft approximation of H, 
\begin{equation*}
\nabla_{\bd{\theta}} L(\bd{\theta}) = \E_{\pi_{\bd{\theta}}(\bd{Z})}[\nabla_{\bd{\theta}}\log \pi_{\bd{\theta}}(\bd{Z})(f(H(\bd{Z}))-\lambda f(S(\bd{Z})))]+ \lambda \E_{\epsilon} [\nabla_{\bd{\theta}} f(S(g(\epsilon, \bd{\theta})))].     \end{equation*}
Let $\pi_{\bd{\theta}}(\bd{W})$ be Bernoulli distribution, then 
\begin{align*}
 \pi_{\bd{\theta}}(\bd{Z})& = 2*\pi_{\bd{\theta}}(H(\bd{Z}))\frac{1}{\sqrt{2\pi}}\exp(-\frac{\bd{Z}^2}{2})  \\
 & = 2*\bd{\theta}^{\frac{H(\bd{Z})+1}{2}}(1-\bd{\theta})^{1-\frac{H(\bd{Z})+1}{2}}\frac{1}{\sqrt{2\pi}}\exp(-\frac{\bd{Z}^2}{2}).
\end{align*}
Let $\bd{U}\sim\mathrm{Uniform}(0, 1),$ $\bd{V}\sim \mathrm{Uniform}(0, 1),$ then $\bd{Z}=\log \frac{\bd{\theta}}{1-\bd{\theta}}+\log\frac{u}{1-u},$ $\bd{W}=H(\bd{Z})$,
$\bd{V}'=(1-\frac{1+\bd{W}}{2})V(1-\bd{\theta})+\frac{1+\bd{W}}{2}(V\bd{\theta}+(1-\bd{\theta})),$
$\wt{Z}=\log \frac{\bd{\theta}}{1-\bd{\theta}}+\log\frac{\bd{V}'}{1-\bd{V}'},$ 
\begin{equation*}
\nabla_{\vthe}L(\vthe) = \E_{p(U, V)}[f(H(Z))- \beta\wt{f}(\sigmoid(Z))\nabla_{\vthe} \log p(W)] +\beta \nabla_{\vthe}(\wt{f}(\sigmoid(Z))-\wt{f}(\sigmoid(\wt{Z}))).    
\end{equation*}

\begin{equation*}
p(W) =\vthe^{\frac{1+W}{2}} (1-\vthe)^{1-\frac{1+W}{2}}
\end{equation*}
\begin {algorithm}[!h]
\caption {Surrogate Model As Control Variates for Training Stochastic BNN}
\label{alg:GF-SVGDonBNN}
\begin {algorithmic}
\small
\Require {training set $\mathbf{X}$ and testing set $\mathbf{X_{test}}$}
\Ensure {Classification accuracy}
\\{\textbf{Initialize} weights $\bd{W}=\sign(\bd{Z})$ with density $p_{\vthe}(W) =\vthe^{\frac{1+W}{2}} (1-\vthe)^{1-{\frac{1+W}{2}}}$.}
\Function{Training}{$\mathbf{X}$}
\For {each epoch}
    \State{Shuffle $\mathbf{X}$}
    \For{iteration $t$}
    \State{$\bd{U}\sim\mathrm{Uniform}(0, 1),$ $\bd{V}\sim \mathrm{Uniform}(0, 1),$ then $\bd{Z}=\log \frac{\bd{\theta}}{1-\bd{\theta}}+\log\frac{u}{1-u},$}
    \State{$\bd{V}'=(1-\frac{1+\bd{W}}{2})V(1-\bd{\theta})+\frac{1+\bd{W}}{2}(V\bd{\theta}+(1-\bd{\theta})),$
$\wt{Z}=\log \frac{\bd{\theta}}{1-\bd{\theta}}+\log\frac{\bd{V}'}{1-\bd{V}'},$ }
    \State{update parameters $\bd{\theta}$ by the following gradient,}
    \State{\begin{equation*}
\nabla_{\vthe}L(\vthe) =\E_X[\E_{p(U, V)}[(f(H(Z),X)- \beta\wt{f}(\sigmoid(Z),X))\nabla_{\vthe} \log p(W)]] +\E_X[\beta \nabla_{\vthe}(\wt{f}(\sigmoid(Z), X)-\wt{f}(\sigmoid(\wt{Z}),X))].    
\end{equation*}}
    \EndFor
\EndFor
\EndFunction\\
\Function{Testing}{$\mathbf{X_{test}}$}
\For{each model $i$}
    \State{Sample $\bd{W}_i=\sign(\bd{Z}_i)$ with learned parameters $\bd{\theta}$ and calculate $f(\mathbf{W}_i,\mathbf{X_{test}})$}
\EndFor
\State{Calculate the ensemble probability $f(\mathbf{W,X_{test}})=\frac1n\sum_{i=1}^{n}f(\mathbf{W}_i,\mathbf{X_{test}})$}
\State{Calculate accuracy using $f(\mathbf{W,X_{test}})$}
\EndFunction
\end {algorithmic}
\end {algorithm}

\section{Simple Rebar}
Let $\bd{W}=\{\bd{W}_i\}_{i=1}^L$ be the binary weight of BNN. The loss function is 
\begin{equation*}
L(\bd{W}; \vthe)=\E_X[\E_{\pi_{\bd{\theta}}(\bd{W})}[f(\bd{W}, X)]]=\E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(H(\bd{Z}), X)]],    
\end{equation*}
where $\bd{W}=H(\bd{Z})=1$ if $\bd{Z}>0$ else $\bd{W}=H(\bd{Z})=-1.$

Consider $\E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(\sigmoid_{\lambda}(\bd{Z}), X)]],$
\begin{equation*}
  \E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(\sigmoid_{\lambda}(\bd{Z}), X)\frac{\partial}{\partial\vthe}\log \pi_{\bd{\theta}}(\bd{Z})]=  \E_X[\E_{\epsilon}[\frac{\partial}{\partial\vthe}f(\sigmoid_{\lambda}(g(\vthe, \epsilon), X)]],  
\end{equation*}

The total one is 
\begin{equation*}
\E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(H(\bd{Z}), X)\frac{\partial}{\partial\vthe}\log \pi_{\bd{\theta}}(\bd{Z})]] -
\beta(\E_X[\E_{\pi_{\bd{\theta}}(\bd{Z})}[f(\sigmoid_{\lambda}(\bd{Z}), X)\frac{\partial}{\partial\vthe}\log \pi_{\bd{\theta}}(\bd{Z})]-\E_X[\E_{\epsilon}[\frac{\partial}{\partial\vthe}f(\sigmoid_{\lambda}(g(\vthe, \epsilon), X)]])   
\end{equation*}
As we use only one sample, we choose $\beta=1.$
% \begin{figure*}
% \begin{tabular}{cc}
% \includegraphics[height=0.44\textwidth]{figs/Acc3000500.pdf}&
% \includegraphics[height=0.44\textwidth]{figs/Loss3000500.pdf}\\
% {\small (a) Accuracy on Training and Test dataset} & {\small (b) Training Loss}
% \end{tabular}
% \caption{Stochastics BNN on Mnist.}
% \end{figure*}


With adaptive weight $w_j = (\frac{\rho(x_j)}{p(x_j)})^{-\beta},$ 
\begin{itemize}
    \item ST + RI is 0.8536 on Alexnet and 0.9130 on VGG with BNN+.
    \item When $\beta=0$, it reduces to SVGD on $\argmax_{\theta} \rho_{\theta}(x)$, the best results is 0.8572.
    \item When $n=1$, SVGD on $\argmax_{\theta} \rho_{\theta}(x)$ is 0.7938.
    \item Sigmoid on activation doesn't work. Only Hardtanh on activation works around .79. Why
\end{itemize}

\section{Straight-Through Estimator}

% \newpage
% \subsection{Using surrogate model as Control Variates}
% Consider Bernoulli r.v. $\theta$ with distribution $\pi_\beta(\theta)=\theta^{\beta}(1-\theta)^{(1-\beta)}$, we want to optimize $L(\beta)= \E_{\pi_\beta}[f(\theta)],$ let $f(\sigma(\theta))$ be the sigmoid function, 
% \begin{equation*}
% \nabla_{\beta} L(\beta) = \E_{\pi_\beta}[f(\theta)\nabla_{\beta}\log \pi_\beta(\theta) - ]       
% \end{equation*}
\newpage
Let $\theta=H(z),$ where $H$ is some hard threshold function. $L(\beta)= \E_{\pi_\beta}[f(\theta)]=\E_{\pi_\beta(z)}[f(H(z))],$
\begin{equation*}
\nabla_{\beta} L(\beta) = \E_{\pi_\beta(z)}[f(H(z))\nabla_{\beta}\log \pi_\beta(z)],       
\end{equation*}
Let $z=g(\epsilon, \beta)=\mu(\beta)+ \epsilon*\sigma(\beta),$ then
\begin{equation*}
\E_{\pi_\beta(z)}[f(\sigmoid(z))] = \E_{\epsilon}[f(\sigmoid(g(\epsilon, \beta)))],    
\end{equation*}
Then we can construct the control variates as
\begin{equation*}
\nabla_{\beta} L(\beta) = \E_{\pi_\beta(z)}[\nabla_{\beta}\log \pi_\beta(z)(f(H(z))-\lambda f(\sigmoid(z)))]+ \lambda \E_{\epsilon} [\nabla_{\beta} f(\sigmoid(g(\epsilon, \beta)))].      
\end{equation*}
Consider $\theta = \mathrm{sign}(z),$ where $z\sim N(\mu, \sigma),$ $\pi_{\beta}(z)= \mathrm{sign}(z)^{\beta}(1-\mathrm{sign}(z))^{(1-\beta)},$ 

Consider $\theta = H(z), $ where $z=g(\epsilon, \beta)=\log \frac{\beta}{1-\beta}+\log \frac{\epsilon}{1-\epsilon},$ $\epsilon \sim \mathcal{U}(0,1),$
% Consider a simple case, where $\theta$ is Bernoulli distribution $\pi_\beta$, $f(\theta)=\mathrm{sign}(\theta),$ 
\subsection{Toy example}
Consider $\theta\in\{-1, 1\},$ $f(\theta)=(\frac{|\theta|+\theta}{2} - 0.49)^2$, $L(\beta)=\E_{\pi_\beta}[(\frac{|\theta|+\theta}{2} - 0.49)^2],$
$\theta = \mathrm{sign}(z),$ where $z=g(\epsilon, \beta)=\log \frac{\beta}{1-\beta}+\log \frac{\epsilon}{1-\epsilon},$ $\epsilon \sim \mathcal{U}(0,1),$
Then 
\begin{equation*}
L(\beta)=\E_{\pi_\beta(z)}[(\frac{|\mathrm{sign}(z)|+\mathrm{sign}(z)}{2} - 0.49)^2]    
\end{equation*}

\begin{figure}[h!]
\centering
\subfigure{\label{fig:stepiter250}
\includegraphics[width=0.45\linewidth]{DiscreteGFSVGD/figs/Variance.pdf}}
\subfigure{\label{fig:stepiter250}
\includegraphics[width=0.45\linewidth]{DiscreteGFSVGD/figs/Losses.pdf}}
\vspace{-0.1in}
\caption{}
\end{figure}

% \begin{figure}[h]
% \begin{tabular}{cc}
% \includegraphics[height=0.44\textwidth]{figs/VGGnet0.pdf}&
% \includegraphics[height=0.44\textwidth]{figs/SVGDalex.pdf}\\
% {\small (a) ST-gradient on VGG and ALex} & {\small (b) GF-SVGD(ranked weights), different particles on VGG net}\\
% \includegraphics[height=0.44\textwidth]{figs/SVGD4.pdf}&
% \includegraphics[height=0.44\textwidth]{figs/SVGD6.pdf}\\
% {\small (c) Compare GFSVGD on Small and Large VGG net }& {\small (d), different Learning rate on 6 particles}\\
% \end{tabular}
% \vspace{-0.1in}
% \caption{Performance on test data. Left Side is VGG Net. The report is 0.89. Right side is GFSVGD with different particle sizes. The accuracy in training data is $0.98\sim 1.0$. Maybe overfitting and try regularization.}
% \end{figure}

==> tex/introduction.tex <==
\section{Introduction}
Discrete probabilistic models provide 
a powerful framework for capturing complex phenomenons and patterns, 
especially in conducting logic and symbolic reasoning. 
However, probabilistic inference of high dimensional discrete distributions such as goodness-of-fit testing and sampling is in general NP-hard and requires highly efficient inference tools.

Traditionally, approximate inference in discrete probabilistic models is performed by Gibbs sampling, Metropolis-Hastings algorithms and deterministic variational approximation, such as belief propagation, mean field approximation and variable elimination methods \cite{wainwright2008graphical, dechter1998bucket}.  
However, these two types of algorithms have their own critical weaknesses: Monte Carlo methods provides theoretically consistent sample-based (or particle) approximation, but are  typically slow in practice, 
while deterministic approximation 
are often much faster in speed, 
but does not provide progressively better approximation like Monte Carlo methods offer. New methods that integrate the advantages of the two methodologies are a key research challenge; see, for example, \cite{liu2015probabilistic, lou2017dynamic, ahn2016synthesis}. 

Goodness-of-fit testing measures how well the model $p(\vx)$ fits observed data $\{\vx_i\}_{i=1}^n$. Classical goodness-of-fit tests includes $\chi^2$ test~\cite{pearson1900x}, the Kolmogorov-Smirnov test~\cite{kolmogorov1933sulla, smirnov1948table} and the Anderson-Darling test~\cite{anderson1954test}. These tests usually assume the model is fully specified and easy to calculate, which cannot be applied to modern complex models with intractable normalization constants.

%is more challenging than continuous graphical models as gradient-based inference algorithms cannot be applied. Metropolis-hastings algorithms, in particular Gibbs sampling, can be applied but are inefficient on large graphical models. Message passing algorithms \cite{wainwright2008graphical} and particles methods such as loopy belief propagation and elimination methods \cite{murphy1999loopy} are applicable for inference on discrete graphical models but lack of convergence guarantees.

Recent computational progress of Stein's method \cite{oates2017control, gorham2015measuring, liu2016stein, chwialkowski2016kernel, gorham2017measuring, chen2018stein, jitkrittum2017linear} provides a practical inference tool on continuous distributions with intractable normalization constant. Kernelized Stein discrepancy (KSD, \cite{liu2016kernelized, chwialkowski2016kernel}) can be applied to test whether \emph{continuous distributions} $p(\vx)$ fits data $\{\vx_i\}_{i=1}^n$ when the gradient of $p(\vx)$ is available. Stein variational gradient descent~(SVGD, \cite{liu2016stein}) integrates deterministic variational inference with sampling for \emph{continuous distributions}. The idea is to directly optimize a particle-based approximation of the intractable distributions by following a functional gradient descent, yielding both practically fast and theoretically consistent algorithms. However, SVGD only works for continuous distributions. An open question is to exploit SVGD for approximate inference of discrete distributions. 

%{\bf Our method} 
In this work, we leverage the power of SVGD and KSD to develop sampling algorithm and goodness-of-fit testing tool on discrete distributions. 
Our idea is to transform discrete distributions to piecewise continuous distributions, on which GF-KSD and GF-SVGD are applied to perform goodness-of-fit testing and sampling respectively. GF-SVGD leverages a differentiable surrogate distribution $\rho(\vx)$ to sample from continuous distributions with unavailable gradient and corrects the induced bias with the importance weight $\rho(\vx)/p(\vx).$ GF-KSD captures a new discrepancy between $q$(data distribution) and the $p$, which replaces the gradient of $p$ in KSD with that of a surrogate $\rho$ and correct the bias with the weight $\rho(\vx)/p(\vx).$  The key challenge in both GF-KSD and GF-SVGD is to design an effective surrogate distribution.

To do so, we design a general framework for transforming discrete distributions to equivalent piecewise continuous distributions, which is specially tailored for our purpose, so that we can conveniently construct effective differentiable surrogates in GF-SVGD and GF-KSD. We investigate the choices of the transform and empirically propose a simple yet effective transform. We apply our proposed algorithms to a wide range of discrete probability models including
Ising models, Bernoulli restricted Boltzmann machines, as well as learning binarized neural networks. We find that our proposed algorithm significantly outperforms 
traditional sampling algorithms for discrete distributions. In particular, our algorithm is shown to provide a promising tool for learning an ensemble of binary neural network (BNN) in which both weights and activation functions are binarized. Learning BNNs has been shown to be a highly challenging problem because standard backpropagation cannot be applied. We cast the task of learning BNN as a Bayesian inference problem of drawing a set of samples (which in turn forms an ensemble predictor) of the posterior of weights,
and apply our SVGD-based algorithm for efficient inference. 
We show that our method outperforms other widely-used ensemble method such as bagging and AdaBoost in achieving  highest accuracy with the same ensemble size and running time on test data. 

On the application of goodness-of-fit testing, our proposed algorithm performs much better than discrete KSD (DKSD, \cite{yang2018goodness}) and maximum mean discrepancy (MMD, \cite{gretton2012kernel}) on benchmark discrete graphical models aforementioned. 

%After transforming the binary-valued  posterior to real-valued one, we relax the non-differentiable posterior to a differetiable approximation as our surrogate when applying our algorithm. We linearly average our learned models for evaluating test accuracy. Our ensemble models interact sufficiently at each iteration during training. At test time, our ensemble method has same cost as other widely-used ensemble method such as bagging and AdaBoost while achieves highest accuracy with the same ensemble size.   

\paragraph{Related work on sampling} 
The idea of transforming 
the inference of discrete 
distributions to continuous distributions have been widely studied, 
which, however, mostly focus on 
leveraging the power of Hamiltonian Monte Carlo (HMC); see, for example,  \cite{afshar2015reflection, nishimura2017discontinuous, pakman2013auxiliary, zhang2012continuous, dinh2017probabilistic, zanella2019informed}. 
Our work is instead motivated by leveraging the power of SVGD, which allows us to derive a novel framework for fast and deterministic sampling for inference of discrete distributions. Our framework of transforming discrete distributions to piecewise continuous distribution is similar to \cite{nishimura2017discontinuous}, 
but is more general and tailored for the application of GF-SVGD. 
Our empirical results show that our method outperforms both traditional algorithms such as Gibbs sampling and discontinuous HMC \cite{nishimura2017discontinuous}. 

\paragraph{Related work on goodness-of-fit test} Our goodness-of-fit testing is developed from KSD \cite{liu2016kernelized, chwialkowski2016kernel} by considering discrete data with unknown distribution and candidate distribution to continuous counterparts. Some forms of goodness-of-fit tests on discrete distributions have been recently proposed such as \cite{martin2017exact, daskalakis2019testing, valiant2016instance}. But they are often model-specialized and require the availability of the normalization constant. \cite{yang2018goodness, gretton2012kernel} is related to ours and will be empirically compared.

%We discuss other related algorithms which can be applied to sample from discrete distributions. continuous parameterization of Hamiltionian Monte Carlo (HMC) \cite{zhang2012continuous} and auxiliary-variable Exact Hamiltonian Monte Carlo Samplers \cite{pakman2013auxiliary} can be applied to sample from discrete distributions. The idea of transforming the discrete probability distributions into a piecewise smooth probability distribution has been explored in the setting of HMC \cite{nishimura2017discontinuous, afshar2015reflection, dinh2017probabilistic}; however, their limitation is that it is difficult to construct HMC proposals relying on numerical methods of a differential equation to maintain volumn-preserving property. 


{\bf Outline} Our paper is organized as follows. Section 2 introduces GF-SVGD and GF-KSD. Section 3 proposes our main algorithms for sampling and goodness-of-fit testing on discrete distributions. Section 4 provides empirical experiments. We conclude the paper in Section 5.

% Discrete distributions and their application are widespread in the world, discrete Markov random field and Ising model are more difficult to inference than continuous ones because of the lack of gradient information. Furthermore, binary neural network (BNN) \cite{courbariaux2016binarized,rastegari2016xnor}, both of whose weights and outputs of each activation function are binary can also not be optimized by truly gradient descent, though it has so many positive qualities such as energy-efficient and memory reduction \cite{fu2018towards}. The same situation is ternary neural networks \cite{mellempudi2017ternary, khan2017lightweight } and other quantized networks \cite{li2017training}. However, endeavors never stops and many approximation methods has been proposed. Gradient estimators are widely used in the back propagation procedure. Straight though estimator \cite{courbariaux2016binarized} and their annealed versions are simple to implement but works well though it is biased. In discrete latent-variable model, a Gumble-softmax distribution \cite{maddison2016concrete,jang2016categorical} can be seen as a continuous relaxations of discrete variables. Policy gradient combined with control variate \cite{tucker2017rebar, grathwohl2017backpropagation} also gives a lower-variance, unbiased gradient estimator which can be applied to a wider variety of problems.

% Different from the devotion to gradient estimator, a recent advance \cite{zhu2018binary} leverages the weakness of binary neural network and combine it with ensemble methods including bagging and boosting, which promotes the accuracy a lot in classification tasks. Similar to their method, our GF-SVGD algorithm also utilize the idea of ensemble. However, instead of naive ensemble methods, our method can consider the weights of each BNN as a particle and construct the corresponding full-precision surrogate by relaxing the sign function to a sigmoid-like function. During training the kernel term can make those particles interactive with each other, which helps optimize the objective function. Binary weights will be finally stored and used during testing.


==> tex/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution
\newcommand{\bd}{\boldsymbol}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/notation.tex <==
\section{Submission of conference papers to ICLR 2019}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2019 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available on the World Wide Web at
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2019_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2019_conference.sty+ and \verb+iclr2019_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2019_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis (as in ``Deep learning shows promise to make progress towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.



==> tex/relatedwork.tex <==

% To tackle the non-differentiable problem of discrete neural network, many approximation methods has been proposed. Gradient estimators are widely used in the back propagation procedure. Straight though estimator \citep{courbariaux2016binarized, hubara2016binarized} and their annealed versions are simple to implement but it is biased. In discrete latent-variable model, a Gumble-softmax distribution \citep{maddison2016concrete,jang2016categorical} can be seen as a continuous relaxations of discrete variables. Actually, these methods have no conflict with ours, on the contrary, all of these gradient estimators can help us construct corresponding surrogate networks whose gradients is exactly those estimators. To further illustrate, our algorithm will degrade to theirs once the number of particles decreases to one.

% Policy gradient combined with control variate \citep{tucker2017rebar, grathwohl2017backpropagation} also gives a lower-variance, unbiased gradient estimator which can be applied to a wider variety of problems. Instead to find a good 'derivative' to a non-continuous function, \citet{shayar2017learning} takes advantage of central limit theorem and local reparameterization trick to model the distribution of pre-activation instead of the distribution of weights. \citet{peters2018probabilistic} also train BNN in a probabilistic way and sample weights when doing test. What's more, \citet{o2016deep} proposed a spiking neural network which looks more like biological brains.

% Recently, an advance \citep{zhu2018binary} leverages the weakness of binary neural network and combine it with ensemble methods including bagging and boosting, which promotes the accuracy a lot in classification tasks. The idea of this method is much more similar to ours except that theirs still use straight through estimator in the back propagation which is biased, while the gradient information we utilize is the exact gradient from differentiable surrogate network. Furthermore, the particles in our algorithm can directly interact with each other during training, which contribute to the optimization.

% An alternative approach to reducing memory requirements and speeding up deep networks utilized weight compression. \citet{louizos2017bayesian,han2015deep} showed that deep networks can be highly compressed without significant loss of precision. However, the speedup capabilities of binary weighted networks, especially on dedicated hardware, is much higher than the compressed one.
